Scribble-Guided Diffusion for Training-free Text-to-Image Generation

Recent advancements in text-to-image diffusion models have demonstrated remarkable success, yet they often struggle to fully capture the user's intent. Existing approaches using textual inputs combined with bounding boxes or region masks fall short in providing precise spatial guidance, often leading to misaligned or unintended object orientation. To address these limitations, we propose Scribble-Guided Diffusion (ScribbleDiff), a training-free approach that utilizes simple user-provided scribbles as visual prompts to guide image generation. However, incorporating scribbles into diffusion models presents challenges due to their sparse and thin nature, making it difficult to ensure accurate orientation alignment. To overcome these challenges, we introduce moment alignment and scribble propagation, which allow for more effective and flexible alignment between generated images and scribble inputs. Experimental results on the PASCAL-Scribble dataset demonstrate significant improvements in spatial control and consistency, showcasing the effectiveness of scribble-based guidance in diffusion models. Our code is available at https://github.com/kaist-cvml-lab/scribble-diffusion.

==> sections/09_dummy.tex <==
\newpage
\quad
\newpage












\MultiDiffusion{
We thoroughly evaluate our method when applied to each task as discussed in Sec. 4. In all experiments, we used Stable Diffusion (Rombach et al., 2022), where the diffusion process is defined over a latent space I = R 64×64×4 , and a decoder is trained to reconstruct natural images in higher resolution [0, 1]512×512×3 . Similarly, the MultiDiffusion process, Ψ is defined in the latent space J = R H‘×W‘×4 and using the decoder we produce the results in the target image space [0, 1]8H0×8W0×3 . We use the public implementation of Stable Diffusion by HuggingFace (von Platen et al., 2022), with the v2 pre-trained model.
}

\DenseDiffusion{
Baselines. We compare our method with various trainingfree methods, which aim to improve the fidelity of the pretrained Stable Diffusion [46] when using dense captions. \\
Composable Diffusion [36] predicts noises for each phrase separately and merges them at every timestep, leading to a longer inference time proportional to the number of phrases. \\
Structure Diffusion [17] employs a language parser to enhance the value features of all parsed phrases at every crossattention layer. eDiffi-Pww [4] manipulates the attention scores for specific query-key pairs according to an additional layout condition. However, since the eDiffi model is not publicly available, we conduct experiments with the Pww implemented on Stable Diffusion (SD-Pww). \\
Metrics. We evaluate each method regarding two criteria: fidelity to the text prompt and alignment with the layout condition. For text prompt, we calculate the CLIP-Score [22], which measures the distance between input textual features and generated image features, and the SOA-I score [23] that uses YOLOv7 [56] to check if the described objects are present in the generated image. In terms of layout alignment, we compare IoU scores of a segmentation map predicted by YOLOv7 [56], with respect to the given layout condition. We further evaluate CLIP-scores on cropped object images (Local CLIP-score [2]) to check whether generated objects followed detailed descriptions. As Composable Diffusion [36] and Structure Diffusion [17] do not take layout conditions, they are excluded for a fair comparison. \\
}


\AaE{
generative semantic nursing
At the core of our method is the idea of \textit{generative semantic nursing}, where we gradually shift the noised latent code at each timestep $t$ toward a more semantically-faithful generation. 
At each denoising step $t$, we consider the attention maps of the subject tokens in the prompt $\mathcal{P}$. Intuitively, for a subject to be present in the synthesized image, it should have a high influence on some patch in the image. As such, we define a loss objective that attempts to maximize the attention values for each subject token. We then update the noised latent at time $t$ according to the gradient of the computed loss. This encourages the latent at the next timestep to better incorporate all subject tokens in its representation. This manipulation occurs on the fly during inference (, no additional training is performed).
In the next sections, we discuss each of the steps presented in for a single denoising timestep $t$ as illustrated in.
}



\BoxDiff{
Conditioning mechanisms in the Stable Diffusion model can explicitly form the cross-attentions between text tokens and intermediate features of the denoiser $\epsilon_{\theta}$. In the denoising step, given the conditioning text tokens $\tau_{\theta}(y)$ and intermediate features $\varphi(x_t)$, the cross-attention $A$ can be accordingly acquired:
\begin{equation}
    A = \text{Softmax}(QK^{\top} / \sqrt{d}),
\end{equation}
% \begin{equation}
%     Q=W_Q \varphi(x_t),\; K=W_K \tau_{\theta}(y),
% \end{equation}
where $Q, K$ are the projection of intermediate features $\varphi(x_t)$ and text tokens $\tau_{\theta}(y)$ by two learnable matrices $W_Q, W_K$, respectively. At each timestep $t$, given $\tau_{\theta}(y)$ with $N$ text tokens $\{athbf{s}_1,\cdots,athbf{s}_N\}$, the cross-attention $A^t$ containing $N$ spatial attention maps $\{A_1^t,\cdots,A_N^t\}$ can be consequently obtained. Here, following~\cite{chefer2023attend}, we remove the cross-attention between the start-of-text token (\emph{i.e.,} \text{[sot]}) and intermediate features before applying Softmax$(\cdot)$. Besides, a Gaussian filter is applied to smooth the cross-attentions along the spatial dimension. Therefore, the aforementioned operations bring an enhancement on cross-attentions between actual subject tokens, \emph{e.g.,} object or context, with the intermediate features. Cross-attention can be performed at different scales, \emph{i.e.,} $64\times 64, 32\times 32, 16\times 16,\text{and } 8\times 8$. Following P2p, we operate the proposed constraints on the cross-attentions with a resolution of $16\times 16$ as the inherent sufficient semantic information. 
}

\CSG{
To formulate constraints on cross-attentions, we begin by detailing the acquisition of attentions and layout information for constraint application. Leveraging latent noise manipulation is pivotal in aligning image-text attentions within designated spatial regions. Drawing on recent research \cite{chefer2023attend,xie2023boxdiff} which suggests that attentions at smaller scales capture semantic information more effectively during early diffusion phases, we employ averaged cross-attentions from user-defined attending objects at the $16 \times 16$ up-scaling block as our manipulation references. Formally, for $N$ attending tokens, we define $\mathcal{A} = \{{A}_i\}_{i=1}^{N}, {A}_i \in \mathbb{R}^{L}$ as the set of cross-attentions relative to the tokens, with $L$ indicating the number of image tokens in cross-attentions. \\
For representing layout information, we employ bounding boxes ${\mathcal{B}} = \{{b}_i\}_{i=1}^N$, which delineate the top-left and bottom-right corner coordinates for each object. Correspondingly, each bounding box ${b}_i$ is transformed into a binary mask ${m}_i$, with pixels inside the box region marked as 1 and those outside as 0. \\
The mask is leveraged in our constraints to discriminate foreground and background pixels of the generation of each object. To mitigate the potential disruption of latent noise's natural Gaussian distribution by gradient-based backpropagation, while ensuring extensive attention coverage within the target region, we employ a \texttt{selective sampling} strategy $\mathcal{F}({m_i})$ for each mask ${m_i}$. Specifically, we select the top $K$ elements within the mask region for focused attention. To avoid concentrating excessively on a limited number of elements, we randomly retain $M$ elements from those selected. 
}


\ShapeGuided{
We present Shape-Guided Diffusion, a \textit{training-free} method that enables a pretrained text-to-image diffusion model to respect shape guidance. Our goal is to locally edit image $x_{src}$ given text prompts $ \mathcal{P}_{src}$ and $ \mathcal{P}_{edit}$ and optional object mask $m$ (inferred from $\mathcal{P}_{src}$ if not provided), so that edited image $x_{edit}$ is faithful to both $\mathcal{P}_{edit}$ and $m$. We introduce Inside-Outside Attention to explicitly constrain the cross- and self-attention maps during both the inversion (image to noise) and generation (noise to image) processes. An overview of our method can be found in and Alg.. We build upon Stable Diffusion (SD), a Latent Diffusion Model (LDM)~\cite{rombach2022high_latent} that operates in low-resolution latent space. LDM latent space is a perceptually equivalent downsampled version of image space, meaning we are able to apply Inside-Outside Attention in latent space via downsampled object masks. For the rest of this paper, when we denote ``pixel'', ``image'', or ``noise'', we are referring to these concepts in LDM latent space.
}




% ----------------------------------------------------------------------------------------------

\DenseDiffusion{
Our goal is to improve the text-to-image model's ability to reflect textual and spatial conditions without fine-tuning.
We formally define our condition as a set of $N$ segments ${\{(c_{n},m_{n})\}}^{N}_{n=1}$, where each segment $(c_n,m_n)$ describes a single region, as shown in Figure.
Here $c_n$ is a non-overlapping part of the full-text caption $c$, and $m_n$ denotes a binary map representing each region. Given the input conditions, we modulate attention maps of all attention layers on the fly so that the object described by $c_n$ can be generated in the corresponding region $m_n$.
To maintain the pre-trained model's generation capacity, we design the modulation to consider original value range and each segment's area.
}


\ControlNet{
ControlNet is a neural network architecture that can enhance large pretrained text-to-image diffusion models with spatially localized, task-specific image conditions. We first introduce the basic structure of a ControlNet in Section 3.1 and then describe how we apply a ControlNet to the image diffusion model Stable Diffusion [72] in Section 3.2. We elaborate on our training in Section 3.3 and detail several extra considerations during inference such as composing multiple ControlNets in Section 3.4.
}


\BoxDiff{
\textbf{Datasets:} Current layout-to-image methods are mainly trained on paired layout-image data of COCO-Stuff caesar2018coco  or VG krishna2017visual. It is unfair to directly make comparisons between our training-free BoxDiff and the fully-supervised methods. Hence, we propose to compare performance on a new dataset. Details can be found in the appendix. Specifically, we collect a set of images (no intersection with COCO and VG) and use YOLOv4 yolov4 to detect objects. For evaluation, we consider two types of situations: i) a single instance, \emph{i.e.,} ``a \{\}"; ii) multiple instances, \emph{i.e.,} ``a \{\}, a \{\}". In this way, 189 different text prompts are combined with conditional boxes for image synthesis. 
\textbf{Evaluation Metrics:} To validate the effectiveness of our BoxDiff, YOLOv4 is employed to detect object-bounding boxes and predict classification scores on the synthesized images. YOLO score, including AP, AP$_{50}$ and AP$_{75}$, is adopted to evaluate the precision of the conditional synthesis. Additionally, we employ a metric of Text-to-Image Similarity (T2I-Sim) to explicitly evaluate the correctness of semantics in the synthesized images. In particular, synthesized images and the text prompts, \emph{e.g.,} ``a photo of \{\}'' or ``a photo of \{\} and \{\}'', are passed to the image and text encoder of pre-trained CLIP, respectively, to calculate their similarity (\emph{i.e.,} T2I-Sim). In CLIP feature space, the similarity can reflect whether the semantics of objects or contexts are correctly presented in the images. 
}



\begin{algorithm}[ht]
\caption{삭제 예정 Scribble-Guided Diffusion}\label{alg:scribble_guided_diffusion}
\textbf{Input:} A diffusion model $DM$ with autoencoder $\mathcal{E}, \mathcal{D}$, real image $x_{src}$, a source prompt $\mathcal{P}_{src}$, an edit prompt $\mathcal{P}_{edit}$, and either a binary object mask $m$ or a shape inference function InferShape$(\cdot)$.\\
\textbf{Hyperparameters:} Timestep interval for scribble propagation $[k_1, k_2]$.\\
\textbf{Output:} An edited image $x_{edit}$ that differs from $x_{src}$ only within the mask region $m$.
\begin{algorithmic}[1]
\If{$m$ is not provided}
    \State $m \gets$ \small{InferShape}($x_{src}, \mathcal{P}_{src}$)
\EndIf
\State $[\bar{z}_0, ..., \bar{z}_T] \sim$ \small{InsideOutsideInversion}$(z | \mathcal{E}(x_{src}), \mathcal{P}_{src}, m, DM)$
\State $z_{T} \gets \bar{z}_{T}$
\ForAll{$t$ from $T$ to $1$} 
    \State \small{InsideOutsideAttention}($DM, \mathcal{P}_{edit}, m$)
    \State $z_{cond} \gets DM(z_{t}, \mathcal{P}_{edit})$
    \State $z_{uncond} \gets DM(z_{t}, \varnothing)$
     \State $z_{t-1} \gets z_{cond} + w_g * (z_{cond} - z_{uncond})$
     \State $z_{t-1} \gets z_{t-1} \odot m + \bar{z}_{t-1} \odot (1 - m)$
\EndFor \\
$x_{edit} \gets \mathcal{D}(z_{0})$
\end{algorithmic}
\label{alg:sgd}
\end{algorithm}



\begin{algorithm}[ht]
    \caption{삭제 예정 Universal Guidance}
    \label{alg:ug}
    \begin{algorithmic}
    \State {\bfseries Parameter:} Recurrent steps $k$, gradient steps $m$ for backward guidance and guidance strength $s(t)$,
    \State {\bfseries Required:} $z_T$ sampled from $\mathcal{N}(0, I)$, diffusion model $\epsilon_{\theta}$, noise scales $\{\alpha_t\}_{t=1}^T$, guidance function $f$, loss function $\ell$, and prompt $c$
    \For{\textit{t} $=T, T-1,\dots,1$}
    \For{\textit{n} $=1, 2, \dots, k$}
    % \State Calculate $\hat z_0$ as \cref{eqn:2}
    \State Calculate $\hat \epsilon_\theta$ using forward universal guidance as guidance 1
    \If {$m > 0$}
    \State Calculate $\Delta z_0$ by minimizing g2 optim with $m$ steps of gradient descent
    \State Perform backward universal guidance by \\ $\hat \epsilon_\theta \gets \hat\epsilon_\theta - \sqrt{\alpha_t/(1 - \alpha_t)} \Delta z_0$ ( g2 guided eps) 
    \EndIf
    \State $z_{t-1} \gets S(z_t, \hat \epsilon_\theta, t)$ 
    \State $\epsilon' \sim  \mathcal{N}(0, I)$ % using N(0,1) in the formula looks a bit awkward to me, so I changed it
    \State $z_t \gets \sqrt{\alpha_t/\alpha_{t-1}} z_{t-1} + \sqrt{1 - \alpha_t/\alpha_{t-1}} \epsilon'$ 
    \EndFor
    \EndFor
    \end{algorithmic}
\end{algorithm}



% ------------------------------------------------------------------------------------------------
% \begin{figure}[!t]
\begin{figure}[ht]
    \centering
    % \includegraphics[width=.95\textwidth]{dummy_figures/Composite_scene_gen.png}
    \includegraphics[width=.95\linewidth]{dummy_figures/Composite_scene_gen.png}
    % \vspace{-0.5em}
    \caption{
        The overall architecture of Scribble.
        Training-free Composite Scene Generation for Layout-to-Image Synthesis (https://arxiv.org/pdf/2407.13609v1)
    }
    \label{fig:overview}
% \vspace{-1.5em}
\end{figure}
% ------------------------------------------------------------------------------------------------


